Dim Silicon and the Case for Improved DVFS Policies

Due to thermal and power supply limits, modern Intel CPUs reduce their frequency when AVX2 and AVX-512 instructions are executed. As the CPUs wait for 670{\mu}s before increasing the frequency again, the performance of some heterogeneous workloads is reduced. In this paper, we describe parallels between this situation and dynamic power management as well as between the policy implemented by these CPUs and fixed-timeout device shutdown policies. We show that the policy implemented by Intel CPUs is not optimal and describe potential better policies. In particular, we present a mechanism to classify applications based on their likeliness to cause frequency reduction. Our approach takes either the resulting classification information or information provided by the application and generates hints for the DVFS policy. We show that faster frequency changes based on these hints are able to improve performance for a web server using the OpenSSL library.

==> Makefile <==
#
#  Makefile
#
#  Execute 'make help' for a list of build targets.
#

target = techreport
#paper_size ?= a4
paper_size ?= letter
pdf_quality ?= printer

all: pdf

##  Rule to generate plot output from the gnuplot input.
plot/%.eps: plot/%.plot
	@echo  "\033[35m$< --> $@\033[0m"
	gnuplot plot/term-eps-nofont.plot $< > $@

plot/%.pdf: plot/%.eps
	@echo  "\033[35m$< --> $@\033[0m"
	epstopdf $< > $@

##  Rules to generate other output
fig/%.eps: fig/%.fig
	@echo "\033[35m$< --> $@\033[0m"
	@fig2dev -L eps -p dummy $< $@

fig/%.eps: fig/%.gif
	@echo  "\033[35m$< --> $@\033[0m"
	@giftopnm $< | pnmtops -noturn -rle > $@

fig/%.eps: fig/%.prn
	@echo  "\033[35m$< --> $@\033[0m"
	@ps2eps -f $<

fig/%.eps: fig/%.ps
	@echo $(EPS)
	@echo  "\033[35m$< --> $@\033[0m"
	@ps2eps -f $<

fig/%.pdf: fig/%.eps
	@echo  "\033[35m$< --> $@\033[0m"
	epstopdf $< > $@

plotclean::
	rm -f plot/*.eps

clean::
	rm -f $(eps_targets) $(pdf_targets) *.eps rev.tex


###########################################################################
eps_targets = $(shell grep '\\epsfig\|\\includegraphics' *.tex | grep -v "\%"  | \
                    sed -e 's/file=//' | sed -e 's/,scale=.*}/}/' | \
                    sed -e 's/.*{\([^{]*\)}.*/\1.eps/;' )
$(target).dvi:: $(target).tex fig/*.tex $(target).bib $(eps_targets)

pdf_targets = $(shell grep '\\epsfig\|\\includegraphics' *.tex | grep -v "\%"  | \
                    sed -e 's/file=//' | sed -e 's/,scale=.*}/}/' | \
                    sed -e 's/.*{\([^{]*\)}.*/\1.pdf/;' )
$(target).pdf:: $(target).tex fig/*.tex $(target).bib $(pdf_targets)

pdf_target = $(addsuffix .pdf, $(target))
ps_target = $(addsuffix .ps, $(target))
dvi_target = $(addsuffix .dvi, $(target))

pdf: $(pdf_target)
ps: $(ps_target)
dvi: $(dvi_target)

help:
	@echo
	@echo "Automatic build target:"
	@echo "    $(pdf_target)"
	@echo "Other build target:"
	@echo "    $(ps_target)"
	@echo

clean = $(target) $(optional)

##############################################################################
#repo =  $(subst .,,$(firstword $(wildcard .git .hg)))
#
#hg_state = $(wildcard .hg/00changelog.i .hg/00changelog.d)
#git_state = $(wildcard .hg/HEAD)
#
#hg.tex: Makefile $(hg_state)
#	@changeset=`hg id | cut -f 1 -d ' '` && echo '\\renewcommand{\Revision}' "{$${changeset}}" > $@
#	-@tipdate=`hg tip | grep "date:" | cut -c 14-44` && echo '\\renewcommand{\RevisionDate}' "{$${tipdate}}" >> $@
#
#git.tex: Makefile $(git_state)
#	@changeset=`git log | head -n1 | cut -d' ' -f2` && echo '\\renewcommand{\Revision}'"{$${changeset}}" > $@
#	-@tipdate=`git log | head -n4 | grep "Date:" | cut -d' ' -f4-8` && echo '\\renewcommand{\RevisionDate}' "{$${tipdate}}" >> $@
#
#rev.tex: $(repo).tex
#	mv $< $@



timezone.tex: Makefile
	-@timezone=`date +%z` && echo '\\renewcommand{\TimeZone}' "{$${timezone}}" > $@

##############################################################################

latex = latex -interaction=batchmode $(1)
pdflatex = pdflatex $(1)
bibtex = bibtex $(1)

gs_screen = -dPDFSETTINGS=/screen
gs_printer = -dPDFSETTINGS=/printer
gs_ebook = -dPDFSETTINGS=/ebook
gs_prepress = -dPDFSETTINGS=/prepress

gs2pdf_options = -dCompatibilityLevel=1.4 $(gs_$(pdf_quality))
gs2pdf = gs -q -dSAFER -dNOPAUSE -dBATCH -sOutputFile=$(1) $(gs2pdf_options) -sDEVICE=pdfwrite -c .setpdfwrite -f $(2)

dvipdfm = dvipdfm -p $(paper_size) -o $(1) $(2)
dvips   = dvips -Pdownload35 -Pcmz -Pcmz -Pamz -t $(paper_size)  -G0 -o $(1) $(2)


RERUN = '(There were undefined references|Rerun to get (cross-references|the bars) right)'
RERUNBIB = 'No file.*\.bbl|Citation.*undefined'
UNDEFINED = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
DVIPDFM_SPECIAL = 'pdf:.*docinfo'


%.pdf: %.tex $(pdf_targets)
	@echo "====> LaTeX first pass"
	$(call pdflatex,$<) || cat $*.log 
	@if egrep -q $(RERUNBIB) $*.log ; then echo "====> BibTex" && $(call bibtex,$*) && echo "====> LaTeX BibTeX pass" && $(call pdflatex, $<) ; fi
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call pdflatex,$<); fi; 
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call pdflatex,$<); fi;
	@echo "====> Undefined references and citations:"
	@egrep -i $(UNDEFINED) $*.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" $*.log || echo "None."


##  Automatically choose the method to convert a DVI into a PDF, favoring
##  dvips since dvipdfm is fragile.
#%.pdf: %.dvi
#	@if egrep -q $(DVIPDFM_SPECIAL) $< ; \
#	 then echo "====> Using dvipdfm" && $(call dvipdfm,$@,$<) ; \
#	 else echo "====> Using dvips" && $(call dvips,$(<:.dvi=.ps),$<) && $(call gs2pdf,$@,$(<:.dvi=.ps)) ; \
#	 fi

##  Build a PDF from PS.  To enable, put this rule before other PDF rules.
#%.pdf: %.ps
#	@echo "====> Converting Postscript to PDF"
#	$(call gs2pdf,$@,$<)

##  Build a Postscript file from the DVI.
%.ps: %.dvi
	@echo "====> Generating Postscript"
	$(call dvips,$@,$<)

%.dvi: %.tex 
	@echo "====> LaTeX first pass"
	$(call latex,$<) || cat $*.log 
	@if egrep -q $(RERUNBIB) $*.log ; then echo "====> BibTex" && $(call bibtex,$*) && echo "====> LaTeX BibTeX pass" && $(call latex, $<) ; fi
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call latex,$<); fi; 
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call latex,$<); fi
	@echo "====> Undefined references and citations:"
	@egrep -i $(UNDEFINED) $*.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" $*.log || echo "None."


clean::
	rm -rf $(addsuffix .pdf, $(clean)) $(addsuffix .ps, $(clean))
	rm -rf $(addsuffix .dvi, $(clean)) $(addsuffix .toc, $(clean))
	rm -rf $(addsuffix .log, $(clean)) $(addsuffix .aux, $(clean))
	rm -rf $(addsuffix .bbl, $(clean)) $(addsuffix .blg, $(clean))
	rm -rf $(addsuffix .out, $(clean))
	rm -rf rev.tex timezone.tex
	rm -rf $(tmp_subdirs)

##############################################################################
#  Additional dependencies
##############################################################################
rev_style = styles/ka-style.sty styles/ibm-style.sty timezone.tex

$(addsuffix .dvi, $(target) $(optional)):: $(rev_style)

##############################################################################
#
#  tex4ht - Renders html from a LaTeX file, using CSS style sheets.
#
#  To build the html output for a given LaTeX file, such as paper.tex,
#  substitute -html for .tex, such as paper-html
# 
##############################################################################

tex4ht ?= ~joshua/tex4ht.dir
tex4ht_bin = $(tex4ht)/bin/unix
tex4ht_styles = $(tex4ht)/texmf/tex/generic/tex4ht

%-html: %.tex FORCE
	mkdir -p $@
	cd $@ && env PATH=$(PATH):$(tex4ht_bin) TEXINPUTS=:..:$(tex4ht_styles) htlatex $<


==> fig/oracle-results.tex <==
\begin{table}[t]
	\begin{center}
		\begin{tabular}{|l|c|c|c|}
			\hline
			Scenario & Instr. & Latency & Freq. \\
			\hline
			\hline
			\multirow{2}{*}{\shortstack[l]{Normal\\ behaviour}} & SSE4 & \SI{732.1}{\micro\second} & \SI{3.1}{\giga\hertz} \\
			\cline{2-4}
			& AVX-512 & \SI{791.5}{\micro\second} (+8.1\%) & \SI{2.4}{\giga\hertz} \\
			\hline
			\shortstack[l]{No frequency\\ changes} & AVX-512 & \SI{637.9}{\micro\second} (-12.8\%) & \SI{3.0}{\giga\hertz} \\
			\hline
			\shortstack[l]{Optimized\\ reclocking} & AVX-512 & \SI{678.9}{\micro\second} (-8.2\%) & \SI{2.95}{\giga\hertz} \\
			\hline
		\end{tabular}
	\end{center}
	\caption{
		TODO
	}
	\label{tab:oracle-results}
\end{table}


